Small Language Models Fine-tuned to Coordinate Larger Language Models improve Complex Reasoning

Large Language Models (LLMs) prompted to generate chain-of-thought (CoT) exhibit impressive reasoning capabilities. Recent attempts at prompt decomposition toward solving complex, multi-step reasoning problems depend on the ability of the LLM to simultaneously decompose and solve the problem. A significant disadvantage is that foundational LLMs are typically not available for fine-tuning, making adaptation computationally prohibitive. We believe (and demonstrate) that problem decomposition and solution generation are distinct capabilites, better addressed in separate modules, than by one monolithic LLM. We introduce DaSLaM, which uses a decomposition generator to decompose complex problems into subproblems that require fewer reasoning steps. These subproblems are answered by a solver. We use a relatively small (13B parameters) LM as the decomposition generator, which we train using policy gradient optimization to interact with a solver LM (regarded as black-box) and guide it through subproblems, thereby rendering our method solver-agnostic. Evaluation on multiple different reasoning datasets reveal that with our method, a 175 billion parameter LM (text-davinci-003) can produce competitive or even better performance, compared to its orders-of-magnitude larger successor, GPT-4. Additionally, we show that DaSLaM is not limited by the solver's capabilities as a function of scale; e.g., solver LMs with diverse sizes give significant performance improvement with our solver-agnostic decomposition technique. Exhaustive ablation studies evince the superiority of our modular finetuning technique over exorbitantly large decomposer LLMs, based on prompting alone.

==> Sections/conclusion.tex <==
\section{Conclusion}
\label{sec:End}

We challenged the design of ever-larger monolithic LLMs as homogeneous network structures, where diverse aspects of problem decomposition and solution are stored in a tangled and opaque manner.
The formidable general-purpose problem-solving capabilities of LLMs are exceedingly resource-hungry, dependent on immense data engineering.
Inspired by brain science, we took a first step toward heterogeneity ---
let two different LLMs evolve independently and adapt to their roles of decomposing and solving complex reasoning problems.
Through extensive experiments on several benchmarks, we showed that such a heterogeneous network can match or exceed some of the largest contemporary LLMs, at a much smaller parameter count. 

% already in limitations
% While \shortname{} is limited to a purely textual guidance to the solver, future endeavors may find further improvements using multimodal and tool-oriented interactions with the solver module.


\clearpage


\section{Limitations}
\label{sec:Limits}

A potential limitation of \shortname, as with many system that uses an LLM-as-a-service API charging per token exchange, is the increased token usage because of the RL exploration.  Asserting a token budget on the decomposer LM is left as an avenue for future exploration.
Ideally, the decomposer LM should seamlessly invoke solvers of many forms, such as retrievers \citep{khattab2022dsp} or mathematical calculators \citep{Toolformer, Wolfram2023ChatGptWolfram}.
Future work may extend \shortname{} to such tools.
\shortname{} is limited to purely text-based subproblem decomposition; it is not possible at present to incorporate reasoning through other modalities (e.g., visual inputs for geometric reasoning) into \shortname{} in its current form.

% SD can continue if you feel like


==> Sections/experiments.tex <==
\section{Experiments}
\label{sec:experiments}



\paragraph{Training data curation.} The training process of \shortname{} consists of two stages as mentioned previously. In the first stage, we require the subproblems along with the reasoning steps for a given problem. We use samples from four existing datasets ---  MATH \cite{MATH}, AQuA \cite{aqua}, GSM8K \cite{gsm8k}, and StrategyQA \cite{StrategyQA}. Each question in these four datasets contains a question \(Q_\text{gold}\), a step-by-step illustration of the reasoning process \(S_\text{gold}\), and the final answer \(A_\text{gold}\). We sample \(7,000\) examples from the training splits of these datasets and employ OpenAI's {\tt text-davinci-003} model  to generate the corresponding subquestions. We provide the model with one-shot example illustrating how to decompose a question into subquestions based on the reasoning. 
In the second stage of training, we utilize the remaining training data from  MATH and AQuA datasets to conduct the policy optimization since this step does not require any supervised examples of subproblems.

\paragraph{LMs used.} We use LLaMA 13 billion \cite{llama} as the decomposer LM. For the solver LM, we primarily use {\tt text-davinci-003} (henceforth, we denote it as {\tt DaVinci} for brevity). We also experiment with the LLaMA 13 bilion and LLaMA 33 billion  models as solvers to test the model-agnostic generalizability of \shortname{}.


\paragraph{Baselines.} We compare \shortname{} with three existing methods of prompting: Chain-of-thought prompting ({\bf CoT})~\citep{CoT}, Least-to-most prompting ({\bf L2M})~\citep{least-to-most}, and Progressive Hint Prompting ({\bf PHP})~\citep{PHP}. The original setting of PHP requires an 8-shot prompting; however, since all other methods including \shortname{} predict in the zero-shot setting, we use PHP in 1-shot for a fairer comparison. Additionally, we experiment on an ablation variant of \shortname{} that does not take the solver feedback into account while generating the subproblems. We specifically finetune this to generate subproblems given the original problem only followed by the policy optimization step. We call this variant \shortname{}-NF.


\paragraph{Test datasets.} For evaluation purposes, we use three datasets -- MATH \cite{MATH}, AQuA \citep{aqua}, and JEEBench \cite{jeebench}. For the first two datasets, only the test splits are used during evaluation since their training splits are used while finetuning the decomposer. The MATH dataset contains mathematical problems on multiple different domains. We report the results on each of them separately and use the following abbreviations -- {\bf ALG}, {\bf I-ALG}, and {\bf P-ALG} for Algebra, Intermediate Algebra, and Pre-Algebra, respectively; {\bf Calc} for Calculus, {\bf Geom} for Geometry, {\bf PnC} for Probability and Combinatorics, {\bf NT} for Number theory. From the JEEBench dataset, we use the problems in Physics ({\bf Phy}) and Mathematics ({\bf Math}). Each of these two subjects has three types of problems -- single-answer multiple-choice questions ({\bf MCQ}), numerical problems ({\bf Num}), and multi-answer multiple-choice questions ({\bf Multi}). For all these datasets, {\em we use exact match criteria to evaluate the correctness of the model-inferred answers}.
%s
Details of training and inference hyperparameters and compute resource usage are provided in Appendix~\ref{hyperparams}.






==> Sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

In recent years, an astounding variety of text and NLP tasks have been accomplished by language models (LMs) \cite{devlin-etal-2019-bert} --- in essence, fitting continuous feature vectors to tokens and modeling smooth conditional distributions over thousands of token positions with multi-task objectives.  
The next generation of large LMs (LLMs) such as T5, GPT4 and \href{https://bard.google.com/}{Bard} \citep{Raffel+2020T5, openai2023gpt4} developed protean capabilities, extending to mathematical and logical ability, based on prompting and in-context learning.
Chain-of-thought (CoT) prompting has been a key enabler \citep{CoT, feng2023CoTexplain}.
LLMs can solve middle-school word problems and equations reasonably well.
It has also acquired the ability to invoke specialized external tools such as Wolfram Alpha \cite{Wolfram2023ChatGptWolfram, Toolformer}.

Recent advances in LLMs have arisen largely from cleverly-engineered, ever-growing training data,
rather than any significant change in network structure,
which remains relatively regular, but with rapidly increasing network size and number of parameters.
One outcome of such giant monolithic LLMs is unsustainable levels of hardware and energy \cite{dhar2020carbon} to train them.
Meanwhile, neurologists and brain scientists have known, via fMRI scans, \emph{inter alia}, that cerebral functions are specialized and spatially localized \cite{Fedorenko2016LanguageAndThought, mahowald2023dissociating}.

Many recent complex reasoning challenges thrown at LLMs have a two-level character --
the input task needs to be decomposed into subtasks, then the subtasks need to be solved,
and finally, subtask solutions have to be consolidated and combined to solve the input task.
Existing approaches use the same LLM to both decompose and solve the task,
sometimes in tangled and uninterpretable ways.
Because sharing an LLM across these functions cannot be closely controlled, very large models are needed for this double ability (decompose and solve) to emerge.

\todo{In fig 1, replace "problem decomposing LM" by "Decomposer LM" done}
\begin{figure*}[t!]
\centering
\includegraphics[width=\textwidth]{Figures/main.pdf}
\caption{{\bf Working example of \shortname{}} on a mathematical reasoning question from the JEEBench dataset~\citep{jeebench}. In this example, the solver LM  is \texttt{text-davinci-003}. In step \button{1}, the solver is prompted to answer the question ({\color{blue} blue} textbox) and it fails to answer correctly ({\color{red} red} textbox). A problem decomposing LM generates subproblems ({\color{violet} violet} textboxes) conditioned on the original question and the initial response of the solver in step \button{2}. In step \button{3}, the solver answers these subproblems iteratively and appends to the prompt. Finally, the original problem is appended to the prompt in step \button{4}, and the solver answers it correctly ({\color{DarkGreen} green} textbox).}
\label{fig:intro-example}
\vspace{-5mm}
\end{figure*}


Staying entirely inside the LLM regime, and avoiding the possibility of specialized tools, we ask a simple question -- \emph{what happens if these two levels of reasoning are entrusted to two different LMs}, each specialized and adapted to its specific function?
Can this model `factoring' enable much smaller LMs to become competitive with giant monolithic LLMs?

\paragraph{Our contributions.}
To study this research question, we develop \shortname{} (\fullname), in which we separate the decomposer from the solver, as shown in Figure~\ref{fig:intro-example}.
The solver LM can be conventionally trained or fine-tuned.  In the illustration, when it answers a question incorrectly, the decomposer LM takes over to produce sub-questions. The partial solutions are appended and resubmitted to the solver LM, which solves the question correctly.
The decomposer LM regards the solver as a black box, and uses reinforcement learning (RL) to become a specialized expert at decomposition, informed by the solver's mistakes.

Extensive experiments with three reasoning datasets (MATH, AQuA, and JEEBench) show that the proposed specialization improves the performance of OpenAI GPT-3 \todo{cite? which major GPT version is this? GPT-3} \texttt{text-davinci-003} to outperform GPT-3.5 and even begins to compete with  GPT-4, outperforming other similar methods. \shortname{} boosts \texttt{text-davinci-003} from an exact match accuracy of \(41.6\) to \(54.5\) in zero-shot regime, which is \(3.9\) points higher than few-shot GPT-4. Similarly, on Physics problems from JEEBench dataset, \shortname{}-augmented {\tt text-davinci-003} scores only \(0.58\) points short of GPT-4 while outperforming GPT-3.5.
The decomposer LM in \shortname{} reduces decomposition errors, and generalizes well across diverse small-scale LMs.  It is also more robust in the face of difficult datasets, where the solver gives near-random performance.

These results support our founding hypothesis that heterogeneous functional specialization improves model efficiency and robustness of LLMs.  We hope this study will inform and guide the design of future foundation networks.\footnote{We commit to release the source code upon acceptance of the paper.}






==> Sections/methods.tex <==
\section{A General Overview of \shortname{}}
\label{sec:prelim}

Given an LM \(\theta\) and a question \( Q\) as a sequence of tokens, a standard zero-shot prompting can be described as, 
\begin{equation*}
\small
    \hat{A} = \argmax_{A \in \mathcal{A}} p_\theta (A|Q)
\end{equation*}
where \(\hat{A}\) is the inferred answer, and \(\mathcal{A}\) is the set of possible answers (e.g., numerical values, multiple-choice options, True/False, etc.). With a CoT prompting, the LM generates a sequence of tokens explaining the steps \(S\) to reach the answer given the question. The modified process \todo{@SD is sum over $S$ the proper abstraction?  also, $S$ may be interleaved with $A$} can be described as,
\begin{equation}
\small
    \hat{A} = \argmax_{A \in \mathcal{A}} \left [ p_\theta (A|S,Q) \argmax_S p_\theta (S|Q)  \right]
    \label{eq:CoT-generation}
\end{equation}

When answering \(Q\) requires multistep reasoning, one can conceptualize \(S\) as a sequence of smaller steps \(\{S'_1, S'_2, \cdots, S'_n\}\) such that the LM iteratively answers a sequence of subproblems \(\{Q'_1, \cdots, Q'_{n}\}\) to finally reach the desired answer to the original question.
Eq.~\ref{eq:CoT-generation} can then be rewritten as,
\begin{equation}
\small
\hat{A} = \argmax_{A'_n \in \mathcal{A}} \hspace{-1mm} \prod_i p_\theta (A'_i|S'_i,Q'_{i}) \argmax_{S'_i} p_\theta (S'_i|Q'_{i})
\label{eq:implicit-substep-CoT}
\end{equation}
where \(A'_i\) is the answer to the subproblem \(Q'_i\). In the usual regime of CoT, the subproblems \(Q'_i\) are implicit; the LM discovers them on its own and generates the reasoning steps and the answers. Due to the repeated multiplication in Eq.~\ref{eq:implicit-substep-CoT}, any error in the initial stages quickly propagates along the chain of steps.

In \shortname{}, we seek to alleviate this problem by offloading the task of inferring the subproblems \(\{Q'_i\}\) to a decomposer LM \(\phi\). For a more guided problem decomposition, \shortname{} uses the answer and the steps generated by the solver LM, \(\theta\) in the naive CoT regime as described in Eq.~\ref{eq:CoT-generation} to generate a set of subproblems \(\{\hat{Q}_i\}_{i=1,\ldots,n}\) as follows:
\begin{align}
\hat{Q}_i = \argmax_{Q'_i} p_{\phi} (Q'_i|&\{\hat{Q}_j: j\in[1,i-1]\}, \notag \\[-2ex]
& Q, \hat{A}_0, S_0),  
% \quad \text{and} 
\label{eq:problem-decompose}
\end{align}
\if 0
\begin{align}
\hat{Q}_i = \argmax_{Q'_i} p_{\phi} (Q'_i|&\{\hat{Q}_j: j\in[1,i-1]\}, \notag \\[-2ex] 
& Q, \hat{A}_0, S_0)
\end{align}
\fi
for $i\in[1,n]$,
where \(\hat{A}_0\) and \(S_0\) are the initial answer and reasoning steps, respectively generated by \(\theta\). The solver LM \(\theta\)  then solves the subproblem set one-by-one similar to Eq.~\ref{eq:implicit-substep-CoT}. However, instead of seeking to generate the final answer as a response to the last subproblem \(\hat{Q}_n\), we append the original question at the end and let \(\theta\) answer it directly given the context generated by the subproblems, their answers, and the corresponding CoTs. The four stages of workflow with \shortname{}, as described in Figure~\ref{fig:intro-example}, can then be summarized as follows:
\begin{equation}
\label{eq:amp-up-final}
\small
    \begin{split}
        &\hat{A}_0 = \argmax_{A \in \mathcal{A}} \left[ p_\theta (A|S_0,Q) \argmax_{S_0} p_\theta (S_0|Q)\right ]\\
        &\hat{Q}_i = \argmax_{Q'_i} p_{\phi} (Q'_i|\{\hat{Q}_j\}_{j\in\{1,i-1\}}, Q, \hat{A}_0, S_0)\\
        &\hat{A}_i = \argmax_{A_i \in \mathcal{A}}\left [ p_\theta (A_i|S_i,\hat{Q}_i) \argmax_{S_i} p_\theta (S_i|\hat{Q}_i)\right ]\\
        &\begin{split}
        \hat{A} = \argmax_{A\in \mathcal{A}}\bigg[
            &p_\theta (A|S, Q)\\ 
            &\argmax_{S} p_\theta (S|\{\hat{A}_i, S_i, \hat{Q}_i\}_{i\in\{1,N\}}, Q) \bigg]
        \end{split}
    \end{split}
\end{equation}

\section{Learning to Decompose from Feedback}
\label{sec:learn-to-decompose}

Typical LMs are not suitable to reliably perform the problem decomposition stage in Eq.~\ref{eq:problem-decompose}. We seek to finetune the decomposer LM, \(\phi\) for this task. Specifically, we use the LLaMA 13 billion model. Instead of full LM-tuning, we use LoRA adapters~\citep{LoRA} for parameter-efficient training. For brevity, we will denote the adapter-augmented LM as \(\phi\), although only the adapter weights are being updated while training. The whole process of teaching the LM to perform the problem decomposition comprises two successive stages: (i) subproblem construction from the original question and CoT, and (ii) policy optimization in conjunction with the solver LM. Details of the supervised data curation required for these three steps are described in Section~\ref{sec:experiments}. Each data sample in the supervised dataset \(\mathcal{D}\) can be conceptualized as a sequence of triplets \(\langle Q_\text{gold}, S_\text{gold}, A_\text{gold}, {\bf Q'}_\text{gold}\rangle\), where \(Q_\text{gold}\) denotes the original question, \(S_\text{gold}\) denotes reasoning steps in form of CoT, \(A_\text{gold}\) denotes the answer to the question, and \({\bf Q'}_\text{gold}\) is a sequence of subproblems generated by decomposing \(Q_\text{gold}\) (see Section~\ref{sec:experiments} and Appendix~\ref{app:SFT_Dataset} for further details on supervised data curation process). 

The first stage is straightforward with the decomposer LM being finetuned using language modeling objective. In the first stage, we seek to optimize the following objective:
\begin{align}
    \min_{\phi} [- \log (p_{\phi}({\bf Q'}_\text{gold}|Q, S))]
\end{align}
This step is somewhat similar to instruction tuning, where an LM is asked to generate some text conditioned on a context, instead of following the usual sentence completion-style behavior of the LM. Intuitively, the role of this stage is to {\em align} the LM to the task of the decomposer.

% {describe in separate paras with headers:
% elements of the environment (observed solver actions, but not differentiable),
% definition of state space of the RL agent,
% definition of action space,
% policy as a function from obs X state to action
% design of policy network
% reward design
% }

\paragraph{Decomposition via policy network.} The previous stage inculcates the ability to decompose a problem within \(\phi\). However, it is still blind to the actual errors made by the solver LM. In the next stage, we seek to make the decomposer LM work in synergy with {\em any} solver LM of choice. This solver agnosticism restrains \(\phi\) to observe the internal representations computed by \(\theta\) while solving the problem. To handle this imposed blackbox characteristics of the solver, we resort to policy gradient optimization of \(\phi\) assuming \(\theta\) to be part of the environment. We formalize the setup as follows.

{\em\bfseries Elements of the environment}: The solver LM \(\theta\) constitutes the core component of the environment. Given a question \(Q\), the solver-generated CoT \(S\) and the answer \(A\) as sequences of tokens define the observation of the policy. 

{\em\bfseries State and action space}: We define the state space as \(\mathcal{S}\). The initial state, \(s_0\in \mathcal{S}\), is defined by the original question \(Q\) and the initial response from the solver, \(S_0, A_0\), that are provided to the decomposer LM \(\phi\) as input. A single timestep is defined on generation of a single token, i.e., the action \(a_t\) at time \(t\). Given the autoregressive nature of LM, we define the state at \(t\)-th timestep as \(s_t = (s_{t-1}, \{a_{t-1}\})\), i.e., the token generated at \(t-1\) appended to the tokens generated till \(t-1\). Trivially, the action space is the same as \(\mathcal{V}\), the vocabulary of \(\phi\).

{\em\bfseries Policy}: The decomposer LM is conceptualized as a policy network \(\pi_{\phi}:\mathcal{S}\xrightarrow{}\mathcal{V}\), i.e., it generates a token given the inputs and the token generated hitherto, till the end of episode \(T\).
Inspired by the recent success in Reinforcement Learning from Human Feedback (RLHF) with autoregressive LMs, we choose the Proximal Policy Optimization (PPO) algorithm to train the policy \(\pi_{\phi}(a|s)\).
In a typical PPO setup, we define the advantage function as follows:
\begin{equation}
\small
    \hat{G}_t = \sum_{i=0}^{T-t+1} (\gamma\lambda)^i\left [r_{t+i}+\gamma V(s_{t+i+1})-V(s_{t+i})\right ]
\end{equation}
where \(r_t\) is the reward at step \(t\), \(V(s_t):\mathcal{S}\xrightarrow{}\mathbb{R}\) is the value function determining the reward associated to state \(s_t\), and \(\gamma, \lambda\) are hyperparameters. We use the policy model augmented with a randomly initialized feedforward layer as the value function. A crucial component in on-policy learning regime is the reward function \(r_t\). While the end goal of the learning is to have the solver answering correctly, the decomposer LM should receive some incremental signal aligned to its generation as well for it to stably converge to the optimal policy. With this goal in mind, we construct the reward function as,
\begin{equation}
    r_t = R_1 + R_2 + R_3 + R_4 + R_5
\end{equation}
where \(R_1\) to \(R_5\) are defined as follows (see Appendix~\ref{app:Reward_details} for a detailed treatment on the reward computation method).
Here $\cossim$ represents cosine similarity. \(I(x)=1\) if \(x\) is true is the indicator function.
%
\begin{description}[leftmargin=1em,noitemsep,topsep=0pt]
\item[Entity coverage:]  \(R_1= \frac{|E_{\bf Q'}|}{|E_Q|}\), where \(E_{\bf Q'}\) and \(E_Q\) are the sets of distinct entities \todo{make sure defined earlier with example} in the generated subproblems and the original question, respectively.

\item[Consistency of answers to subproblems:] 
\begin{equation}
\small
R_2 = 
\sum_i \big(I({e_i} = {\hat{e_i}}) + \cossim(Q'_i, A_i)\big)
\end{equation}
%\todo{cos can be negative, how about $\sigma(\cos(\cdot))$ or $(1+\cos(\cdot))/2$} 
where \(\hat{e_i}\) is the entity whose value has been asked in the subproblem \(Q'_i\), and \({e_i}\) is the entity answered. This reward penalizes the decomposer LM for generating questions whose answers are not consistent.

\item[Order of operations:]  $R_3 = \frac{l}{m}$, where $l$ is the number of operations matched in order between \(S\) and \(S_\text{gold}\), and $m$ is the total number of operations in \(S_\text{gold}\).

\item[CoT proximity:] To ensure that the distance of reasoning produced by the model after prompting \(S\) to the gold reasoning \(S_{gold}\) is less than the distance of reasoning produced without prompt \(S_0\) to the gold reasoning steps \(S_{gold}\), we design a reward based on the cosine similarity of each step of  \(S_{gold}\). We break \(S\) and \(S_0\) at new-line token to form reasoning steps. At each step $j$, we compute  $c_{1j} = \cossim(S^j, S_{gold}^j)$ and $c_{2j} = \cossim(S_0^j, S_{gold}^j)$. The reward is
\begin{equation}
\small
R_4 = \sum_{j=0}^{m} I(c_{1j}>c_{2j})c_{1j} + 
I(c_{2j}>c_{1j})(-1-c_{2j}),  
\end{equation}

\item[Correctness of final answer:] $R_5{=} I(\hat{A}{=}A_\text{gold})$.
\end{description}
%
Now, we can define the PPO objective as follows:
\begin{equation}
\label{eq:ppo-objective}
\small
    \max_{\phi} \left(\mathbb{E}_t\left [\frac{\pi_\phi (a_t|s_t)}{\pi_\text{ref} (a_t|s_t)}\hat{G}_t\right] - \beta \mathbb{E}_t\left [K_t\right] \right )
\end{equation}
where \(\pi_\text{ref}\) is the reference model that is initialized with supervised finetuned \(\phi\). \(K_t = \operatorname{KL}[\pi_\text{ref}(\cdot|s_t), \pi_{\phi}(\cdot|s_t)]\) is the KL-divergence between the reference model and the policy model. 

The resulting decomposer LM \(\phi\) optimized using the above mentioned three stages of finetuning can then be used with \shortname{}.

==> Sections/related_work.tex <==
\section{Related Work}
\label{sec:rw}

Eliciting superior reasoning abilities in LM through specially designed prompts has found its popularity through CoT prompting~\cite{CoT} -- asking the LM to explain the reasoning steps improves overall performance. Decomposing a complex reasoning requirement into multiple, simple steps results in superior reasoning capabilities across modalities other than free-form natural language text as well, e.g., reasoning over tabular data~\citep{decompose-tabular}, visual question answering~\cite{CoT-vqa}, etc. These methods generally solicit a single run of LM inference with no intermediate prompting interactions. Consequently, the LM often misses key reasoning steps or hallucinates irrelevant ones.

On the other hand, a prototypical prompter, sequentially interacting with the LM, has shown impressive performance. Progressive Hint Prompting \cite{PHP} uses such a setting; first, the LM is asked to provide a base answer. The prompt then uses the answer as a hint to the LM that progressively guides it to the final answer. \citet{least-to-most} followed a similar direction by breaking down the problem itself. Their method, Least-to-most prompting, asks the LM to generate simpler, related problems from a complex problem. The final solution to the original question is generated by the LM conditioned upon the solution of the subproblems. A major bottleneck then becomes the solver's ability to identify the critical subproblems. Decomposing a complex task and then solving each task via multiple LLMs with their own in-context examples have been attempted as well~\citep{successive, khot2023decomposed}. Recently, \citet{shridhar2022distilling} explored subquestion generation from complex questions as means of distilling reasoning abilities from larger LMs to smaller ones. 

Our proposed method, \shortname{} makes a departure from these mentioned approaches in three particular features: (i) we seek to separate out the decomposer from the solver to get rid of the solver's limitations affecting decomposition, (ii) the decomposer acts as a plug-and-play module that can generalize to any solver, and (iii) the decomposition actuates with complete knowledge of the solver's actions.



==> Sections/results.tex <==
\section{Experimental Results}
\label{sec:results}
The tasks used to evaluate the performance of \shortname{} contain questions that can be answered either of the three types -- numerical, single correct answer MCQ, and multiple correct answer MCQ. %{\em In all cases, we evaluate using exact match criteria}. 

\begin{table}[!t]
\centering
\adjustbox{max width=\hsize}{ \tabcolsep 3pt
\begin{tabular}{l|c|c|c||c|c}
\hline
%      Method          & PnC & NT   & ALG  & iALG & Cal   &    PAlg & Geom & AQuA \\
%     \hline
%     CoT             & 16.4 & 14.4 & 27.6 & 16.4 & 14.0  &   32.3  &   14.2   &41.6\\
%     L2M             & 16.0 & 11.0 & 22.4 & 16.8 & 14.58 &   28.0  &   12.5   &44.7\\
%     PHP-1shot       & 10.2 & 9.8  & 24.0 & 10.0 & 14.28 &   26.5  &   14.0   &44.4\\
%     \shortname{}-NF & 20.0 & 18.4 & 31.6 & 20.8 & 15.1  &   38.0  &    19.04  & 53.2\\
% \shortname{}        & \textbf{21.4} & \textbf{26.1} & \textbf{33.4} & \textbf{24.8} & \textbf{18.2} & \textbf{44.0} & \textbf{21.4} &\textbf{54.5}\\
%     \hline
    \multirow{2}{*}{Dataset} & \multicolumn{5}{c}{Method} \\\cline{2-6}
    & CoT & L2M & PHP & \shortname{}-NF & \shortname{}\\
    \hline
    PnC & \(16.4\) & \(16.0\) & \(10.2\) & \(20.0\) & \(\bf 21.4\) \\
    NT & \(14.4\) & \(11.0\) & \(9.8\) & \(18.4\) & \(\bf 26.1\) \\
    ALG & \(27.6\) & \(22.4\) & \(24.0\) & \(31.6\) & \(\bf 33.4\) \\
    I-ALG & \(16.4\) & \(16.8\) & \(10.0\) & \(20.8\) & \(\bf 24.8\)\\
    Calc. & \(14.0\) & \(14.58\) & \(14.28\) & \(15.1\) & \(\bf 18.2\) \\
    P-ALG & \(32.3\) & \(28.0\) & \(26.5\) & \(38.0\) & \(\bf 44.0\) \\
    Geom. & \(14.2\) & \(12.5\) & \(14.0\) & \(19.04\) & \(\bf 21.4\) \\
    \hline
    AQuA & \(41.6\) & \(44.7\) & \(44.4\) & \(53.2\) & \(\bf 54.5\) \\
    \hline
\end{tabular}}
\caption{Performance comparison on  MATH and AQuA datasets using {\tt DaVinci} as the solver LM. See Section \ref{sec:experiments} for abbreviations.}
\label{tab:gpt-table-1}
\vspace{-5mm}
\end{table}

% \begin{table}[!t]
% \centering
% \footnotesize
% \scalebox{0.7}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
%      Method          & PnC & NT   & ALG  & iALG & Cal   &    PAlg & Geom & AQuA \\
%     \hline
%     CoT             & 16.4 & 14.4 & 27.6 & 16.4 & 14.0  &   32.3  &   14.2   &41.6\\
%     L2M             & 16.0 & 11.0 & 22.4 & 16.8 & 14.58 &   28.0  &   12.5   &44.7\\
%     PHP-1shot       & 10.2 & 9.8  & 24.0 & 10.0 & 14.28 &   26.5  &   14.0   &44.4\\
%     \shortname{}-NF & 20.0 & 18.4 & 31.6 & 20.8 & 15.1  &   38.0  &    19.04  & 53.2\\
% \shortname{}        & \textbf{21.4} & \textbf{26.1} & \textbf{33.4} & \textbf{24.8} & \textbf{18.2} & \textbf{44.0} & \textbf{21.4} &\textbf{54.5}\\
%     \hline
    
% \end{tabular}}
% \caption{Comparison on MATH and AQuA datasets using {\tt Davinci} as the solver LM (NF: problem decomposition without feedback).}
% \label{tab:gpt-table-1}
% \end{table}


\begin{SCtable*}
\centering
 \small
\begin{tabular}{l|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{8}{c}{Dataset} \\\cline{2-9}
    & PnC & NT & ALG & iALG & Geom & Cal & Palg & AQuA \\
    \hline
    \multicolumn{9}{c}{LLaMA 13 billion} \\
    \hline
    CoT              &2.05  & 4.0  & 3.12  &  2.4 & 3.2 & 2.08 & 5.0 &17.7\\
    L2M              & 1.66 & 3.2  & 3.33  &  2.8 & 2.0 & 3.33 & 4.54 & 16.6\\
    \shortname{}-NF  &2.93  & 4.8  & 4.68  &  3.2 & 4.0 & 3.9 & 6.2 &21.6\\
    \shortname{}     & \textbf{4.0}  & \textbf{5.6}  & \textbf{4.70} & \textbf{ 3.4} & \textbf{4.3} & \textbf{4.1}& \textbf{8.33}&\textbf{22.0}\\
    \hline
    \multicolumn{9}{c}{LLaMA 33 billion} \\
    \hline
    CoT  & 2.4  & 4.16 & 4.54 &  3.7 & 4.0& 4.0 & 5.2 & 20.0\\
    L2M &  2.38 & 4.16 & 4.2 &  6.0 & 4.25 & 5.71 & 5.55& 21.6 \\
    \shortname{}-NF  & 3.2  & 5.83 & 5.6  &  5.6 & 5.1 & 5.71 & 5.2&22.5\\
    \shortname{}   & \textbf{4.0 } & \textbf{7.36} & \textbf{9.09} &\textbf{ 6.02} &\textbf{5.3} & \textbf{6.03}& \textbf{8.44}&\textbf{ 26.8}\\
    
    \hline
\end{tabular}
\caption{Performance on MATH and AQuA with LLaMA 13 billion and LLaMA 33 billion as solvers. PHP is not reported as one-shot PHP generated randomly with both LLaMA variants. Base CoT performs pretty poorly across all tasks in MATH, and L2M is mostly unable to improve upon this. \shortname{} provides consistent improvement across all the tasks.}
\label{tab:llama-results}
\end{SCtable*}


\begin{table*}[!t]
\centering
\footnotesize
\begin{tabular}{l|c|c|c|c|c|c|c|c}
    \hline
    \multirow{2}{*}{Method} & \multicolumn{8}{c}{Dataset} \\\cline{2-9}
    & Phy MCQ & Math MCQ & Phy Multi & Math Multi & Phy Num & Math Num & Phy Int & Math Int  \\
     \hline
     CoT & 33.33 & 21.9 & 6.25 &12.0 & 3.03&1.69 &12.5 &20.0\\ 
     PHP & 22.22& 17.07	& 6.25	&	7.59 &3.03	& 1.69	&	0*&	 4.0\\ 
     L2M & 22.22&	21.9&	6.25&	12.5&	3.03&	3.38&	10.0&	20.0\\ 
     \shortname{}-NF & 20.8 &31.7 & 7.5	& 10.12 &3.03	& 3.38&12.5 &16.0\\
     \shortname{} & \textbf{55.55} & \textbf{36.5}	& \textbf{18.75}&\textbf{ 16.0}& 	\textbf{6.06} & \textbf{10.16}&  \textbf{22.5}& \textbf{24.0}\\ 
     \hline     
\end{tabular}
    \caption{Performance comparison on the JEE benchmark dataset with {\tt DaVinci} as the solver LM. 0* signifies that the model was not able to answer any problem in the task correctly.}
    \label{tab:jeebench}
    \vspace{-5mm}
\end{table*}



\paragraph{\shortname{} is better than vanilla CoT.} We start with \shortname{} augmented with {\tt DaVinci} as the solver LM on MATH and AQuA datasets (see Table~\ref{tab:gpt-table-1}). The improvement achieved with \shortname{} prompting compared to standard CoT is staggering across all types of problems in the MATH dataset: \(+11.7\) on Pre-Algebra, \(+8.4\) on Intermediate Algebra, \(+7.7\) on Number Theory, \(+7.2\) on Geometry, \(+5.0\) on Probability and Combinatorics, \(+5.8\) on Algebra, and \(+4.2\) on Calculus. The absolute improvement is even larger on the AQuA dataset, i.e., \(+12.9\) over CoT. It is noticeable that the effects of \shortname{} are stronger across tasks containing algebraic reasoning (AQuA, Pre- and Intermediate-Algebra, etc.) compared to Probability and Combinatorics or Calculus, which require more implicit knowledge. 

\paragraph{\shortname{} is better than pure prompting methods.} The performance gain achieved via \shortname{} is significantly better compared to methods like L2M or PHP. The latter methods often fail to improve over standard CoT (e.g., on Probability and combinatorics, Number Theory, and Algebra problems, L2M shows a drop in accuracy). Even when improving over CoT, their improvement is meager compared to \shortname{}. This trend entails our earlier argument in support of offloading the problem decomposition task to a specialized LM; methods that prompt the solver LM to decompose the problem lack the expertise achieved via dedicated finetuning in \shortname{}.

\paragraph{Feedback from the solver is important.} 

In the preceding paragraph, we attributed the superiority of \shortname{} over other methods to the usage of a specialized LM for problem decomposition. However, manipulating the problem decomposition upon feedback from the solver is also an important factor here. None of the existing methods does so, and therefore, remains blind towards what reasoning (and possible errors) is followed by the solver model. 
This is further manifested when we compare \shortname{} with itself without the feedback module, \shortname{}-NF. While \shortname{}-NF is able to improve upon basic CoT and other prompting methods, it falls short of the regime when the problem decomposing LM has access to the initial response of the solver. 



\paragraph{\shortname{} generalizes to smaller solvers.} An important aspect of a prompting method is its ability to work with LMs of different scales. Despite being finetuned with {\tt DaVinci} responses only, \shortname{} is able to improve upon the base performance of smaller scale LLaMA models as well (see Table~\ref{tab:llama-results}). L2M prompting generally fails with both LLaMA 13 billion and 33 billion variants. On the other hand, \shortname{}, with or without feedback, almost doubles the performance of the base CoT  across multiple tasks of the MATH dataset. It shows substantial improvement on AQuA as well. However, the importance of feedback from the solver LM usually manifests strongly in proportion to the scale of the solver.

\paragraph{\shortname{} generalizes to harder problems.} Since the decomposer LM \(\phi\) is trained using a subset of the training data of MATH and AQuA, we opt for a harder (in terms of benchmark performance of different LMs) reasoning evaluation on the JEEBench dataset. Table~\ref{tab:jeebench} summarizes the performance of the baselines and \shortname{} with {\tt DaVinci} as the solver LM on Mathematics and Physics questions of the JEEBench dataset. We notice that the superiority of \shortname{} manifests even more profoundly on this task compared to the former ones. Both PHP and L2M prompting absolutely fail to improve upon basic CoT prompting, often with a sharp fall in performance (e.g., Physics MCQ questions). On the other hand, \shortname{} boosts the LMs performance, very often over 100\% relative improvement (all three types of problems in Physics and numerical problems in Mathematics). Aggregated across question types, \shortname{} boosts the performance of {\tt DaVinci} to \(22.420\) in Physics and \(22.07\) in Mathematics. It is noteworthy that the same LM in its base setting performs near-random, i.e., \(10.4\) and \(10.7\) in Physics and Mathematics, respectively, whereas a random selection baseline gives scores of \(9.6\) and \(10.3\), respectively~\citep{jeebench}. Furthermore, {\tt DaVinci} with \shortname{} outperforms a better optimized candidate of the GPT series, GPT-3.5 on both these subjects (note that \citet{jeebench} reported \(18.9\) and \(15.7\) scores with GPT-3.5 on Physics and Mathematics, respectively). 

\paragraph{Comparison with GPT-4.} The colossal compute used by GPT-4 makes the comparison with any of its predecessors like {\tt DaVinci} quite unfair. However, it is tempting to observe that \shortname{} boosts the performance of {\tt DaVinci} often to the level of GPT-4. For example, on arithmetic problems of the AQuA dataset, \shortname{} surprisingly outperforms both zero-shot and few-shot GPT-4 (\(40.6\) and \(50.4\) respectively, compared to \(54.5\) with {\tt DaVinci} and \shortname{}). On MATH dataset, \shortname{} augmented {\tt DaVinci} scores an aggregate of \(30.23\), which is better than ChatGPT (\(26.4\)) and close to GPT-4 (\(35.7\)). On JEEBench Mathematics problems, GPT-4 comes up with a score of \(23.1\), which is pretty close to our \(22.42\). These results definitely do not claim any assumed superiority of \shortname{}-boosted {\tt DaVinci} over GPT-4 since there are multiple other cases that state otherwise. Instead, we seek to demonstrate how much leftover potential these LMs possess that can be unleashed via our proposed method of feedback-guided automatic problem decomposition.
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{Figures/Example 1.pdf}
    \caption{An example case study on a problem from the MATH dataset. {\tt DaVinci} is used as the solver LM with three different methods of prompting -- standard CoT, Least-to-most, and \shortname{}. Only \shortname{} is able to guide the model to the correct answer.}
    \label{fig:case-study}
    % \vspace{-3mm}
\end{figure*}

\section{Case Study} To this point, we have compared the numbers produced by \shortname{}-boosted models across different datasets. While they provide an overall assessment, deeper analyses are needed to comprehend the actual reasoning steps adopted by these different methods.  Figure~\ref{fig:case-study} shows the reasoning steps generated by {\tt DaVinci} given an example problem from the MATH dataset with three different prompting methods -- vanilla CoT, L2M, and \shortname{}. Note that \shortname{} uses the CoT output to decompose the problem.

Both CoT and L2M end up with the model answering incorrectly. With CoT, the solver wrongly assumes that the given equation must have two real roots though it should not have any real roots. Also, it mistakes the value of \(a^2\) as \(a\). The effect is prominent in the subproblems generated by \shortname{} as it asks to find the value of \(a\) explicitly. Furthermore, the solver LM specifically announces that \(y\leq 0\) to  answer the first subproblem generated by \shortname{}. This helps to correct the reasoning about the sign of the discriminant. 

With L2M, the confusion around the value of \(a\) and \(a^2\) persists, as the solver LM substitutes \(a\) in the given equation by \(49\) (which is the value of \(a^2\)) twice in the answering process. Although it substituted the correct value of \(a\) once while answering the second question, it is not explicitly declared like in \shortname{}. We observe multiple similar failure cases with L2M. It is quite likely that prompting the model to generate the final answer after each subproblem accumulates the erroneous reasoning steps that the model falls prey to.



With \shortname{}, the reasoning steps followed by the solver remains robust throughout. In fact, it reaches the final answer much earlier (third and fourth subproblems). In the final answer, the solver simply reiterates the steps that it earlier generated to answer the subproblems. This is a common behavior that we observed across multiple problems from multiple datasets. In Appendix~\ref{llama-examples} (see Figures~\ref{fig:llama-case-13b} and \ref{fig:llama-case-33B}), we provide similar case studies on LLaMA 13 billion and LLaMA 33billion with different prompting methods. With reduced solver capacity, the difference between Least-to-most and CoT generated reasoning steps further diminishes with both leading to incorrect answers; \shortname{}, on the other hand, still guides the solver through correct steps.

An interesting observation can be made by comparing how the solver behaves with CoT vs. with \shortname{}. With \shortname{}, we do not provide any new knowledge to the solver. Yet, the same model can rectify its errors made in CoT response. This may point to the intuition that current LLMs are actually underutilized, and one can unfold even more impressive performance with cleverly composed guidance. 
